A DRL Approach for RIS-Assisted Full-Duplex UL and DL Transmission: Beamforming, Phase Shift and Power Optimization

We propose a deep reinforcement learning (DRL) approach for a full-duplex (FD) transmission that predicts the phase shifts of the reconfigurable intelligent surface (RIS), base station (BS) active beamformers, and the transmit powers to maximize the weighted sum rate of uplink and downlink users. Existing methods require channel state information (CSI) and residual self-interference (SI) knowledge to calculate exact active beamformers or the DRL rewards, which typically fail without CSI or residual SI. Especially for time-varying channels, estimating and signaling CSI to the DRL agent is required at each time step and is costly. We propose a two-stage DRL framework with minimal signaling overhead to address this. The first stage uses the least squares method to initiate learning by partially canceling the residual SI. The second stage uses DRL to achieve performance comparable to existing CSI-based methods without requiring the CSI or the exact residual SI. Further, the proposed DRL framework for quantized RIS phase shifts reduces the signaling from BS to the RISs using $32$ times fewer bits than the continuous version. The quantized methods reduce action space, resulting in faster convergence and $7.1\%$ and $22.28\%$ better UL and DL rates, respectively than the continuous method.

==> fig/basestation.tex <==

% chktex-file 1
% chktex-file 27

\makeatletter


% The keys that the user can provide are all the keys below.

% Keys for the Beam shape
\pgfkeys{
  /pgf/.cd,
  % The 4 following options control the proportion of shapewidth/shapeheight for
  % the control points of the beam -> The must be greater than zero
  control point 1 x/.initial=0.35,
  control point 1 y/.initial=1.0,
  control point 2 x/.initial=0.5,
  control point 2 y/.initial=0.25,
}

% Keys for the UserTerminal shape
\pgfkeys{
  /pgf/.cd,
  button fill color/.initial=white,
  screen fill color/.initial=white,
}


% Represents a "beam", which is constructed using two Bézier curves.
% The two control points can be controlled by passing the
% "control point 1 x/control point 1 y/control point 2 x/control point 2 y"
% parameters.
\pgfdeclareshape{Beam}{

  % xxxxxxxxxx Define some saved macros xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \savedmacro\shapewidth{
    \def\shapewidth{\pgfkeysvalueof{/pgf/minimum width}}
  }

  \savedmacro\shapeheight{
    \def\shapeheight{\pgfkeysvalueof{/pgf/minimum height}}
  }

  \savedmacro\firstpointxprop{
    \def\firstpointxprop{\pgfkeysvalueof{/pgf/control point 1 x}}
  }
  \savedmacro\firstpointyprop{
    \def\firstpointyprop{\pgfkeysvalueof{/pgf/control point 1 y}}
  }
  \savedmacro\secondpointxprop{
    \def\secondpointxprop{\pgfkeysvalueof{/pgf/control point 2 x}}
  }
  \savedmacro\secondpointyprop{
    \def\secondpointyprop{\pgfkeysvalueof{/pgf/control point 2 y}}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \savedanchor\startpoint{%
    \pgfmathsetlength\pgf@x{-0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  \savedanchor\endpoint{%
    \pgfmathsetlength\pgf@x{0.5*\shapewidth}
    \pgfmathsetlength\pgf@y{0}
  }

  % \savedanchor\centerpoint{%
  %   \pgf@x=0%
  %   \pgf@y=0%
  % }

  % Control point anchors
  \savedanchor\firstcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointtop{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{\secondpointyprop*\shapeheight}
  }

  \savedanchor\firstcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\firstpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\firstpointyprop*\shapeheight}
  }

  \savedanchor\secondcontrolpointbottom{%
    \pgfmathsetlength\pgf@x{\secondpointxprop*\shapewidth}
    \pgfmathsetlength\pgf@y{-\secondpointyprop*\shapeheight}
  }

  % xxxxxxxxxx Define regular anchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{center}{\startpoint}
  \anchor{start}{\startpoint}
  \anchor{end}{\endpoint}
  \anchor{main region}{
    \endpoint
    \pgfmathsetlength\pgf@x{\pgf@x-0.25*\shapewidth}
  }
  \anchor{top control point 1}{\firstcontrolpointtop}
  \anchor{top control point 2}{\secondcontrolpointtop}
  \anchor{bottom control point 1}{\firstcontrolpointbottom}
  \anchor{bottom control point 2}{\secondcontrolpointbottom}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  \inheritanchorborder[from=rectangle]

  % xxxxxxxxxx Draw the background path xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    \begin{pgfscope}
      \pgfmoveto{\startpoint}
      \pgfcurveto{\firstcontrolpointtop}{\secondcontrolpointtop}{\endpoint}
      \pgfcurveto{\secondcontrolpointbottom}{\firstcontrolpointbottom}{\startpoint}
      \pgfpathclose
      \pgfusepath{fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx UserTerminal Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{UserTerminal}{

  % xxxxxxxxxx First we define some savedmacros xxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Macros and savedanchors common to UserTerminal and BaseStation Shapes
  \savedanchor{\center}{
    \pgf@x=0pt
    \pgf@y=0pt
  }

  % Note that pgf provides the text macros \pgfshapeminwidth and
  % pgfshapeminheight that store the minim width and minimum height,
  % respectivelly. Note that They are "TEXT macros" and not
  % "lengths". Calling them simple
  % replaces for the text.
  \savedanchor{\northeast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
    % NOTE: We can't use 0.5\pgfshapeminwidth directly because the minimum
    % width is stored in a "plain text macro". If minimum width is 2cm, for
    % instance, and we write "\pgf@x=.5\pgfshapeminwidth" then \pgf@x would
    % be set to 0.52cm, which is not what we want. See the explanation for
    % \savedanchor in the pgfmanual (page 627).
  }

  \savedanchor{\southwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=-0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Savedanchors specific to the UserTerminal shape
  \savedanchor{\screennortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.45\pgf@xa
    \pgf@y=0.45\pgf@ya
  }

  \savedanchor{\screensouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.45\pgf@xa
    \pgf@y=-0.35\pgf@ya
  }

  \savedanchor{\buttonsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by -0.15\pgf@xa
    \advance\pgf@y by -0.04\pgf@ya
  }

  \savedanchor{\buttonnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=-0.425\pgf@ya
    \advance\pgf@x by 0.15\pgf@xa
    \advance\pgf@y by 0.04\pgf@ya
  }

  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from rectangle xxxxxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=rectangle]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from rectangle xxxxxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % rectangle shape (even thought the northeast and southwest saved anchors
  % in the rectangle shape are different from ours).
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Now we define more regular anchors xxxxxxxxxxxxxxxxxxxxxxxxx
  \anchor{text}
  {
    % This will get the center of the screen
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
    % Lets put the center of the text in the center of the screen
    \advance\pgf@x by -0.5\wd\pgfnodeparttextbox
    \advance\pgf@y by -0.5\ht\pgfnodeparttextbox
  }

  \anchor{button}{
    \pgfpointlineattime{0.5}{\buttonsouthwest}{\buttonnortheast}
  }

  \anchor{screen}{
    \pgfpointlineattime{0.5}{\screensouthwest}{\screennortheast}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \backgroundpath{
    % Scope for Terminal Body
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      % '\pgfshapeminheight' cannot be used directly; or if you want to use it directly use the '*' for multiplication
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfpathrectanglecorners
      {\southwest}
      {\northeast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the terminal Screen
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.03\pgf@ya}{0.03\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/screen fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\screensouthwest}
      {\screennortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the button
    \begin{pgfscope}
      \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
      \pgfsetcornersarced{\pgfpoint{0.009\pgf@ya}{0.009\pgf@ya}}
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/button fill color}}
      %\pgfsetfillcolor{white}
      \pgfpathrectanglecorners
      {\buttonsouthwest}
      {\buttonnortheast}
      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStationSimple xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStationSimple}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from UserTerminal. We only need northeast and
  % southwest, but we can't choose which ones to inherit.
  \inheritsavedanchors[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.12\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.12\pgf@xa
  }

  % Maybe I don't need this savedanchor
  \savedanchor{\MiddleAntennasouth}{
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0pt
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\AntennaConnectorsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.38\pgf@ya
  }

  \savedanchor{\AntennaConnectornortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.42\pgf@ya
  }

  \savedanchor{\MiddleAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.15\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\MiddleAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.15\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\LeftAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.5\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\LeftAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=-0.25\pgf@xa
    \pgf@y=0.5\pgf@ya
  }

  \savedanchor{\RightAntennasouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.25\pgf@xa
    \pgf@y=0.29\pgf@ya
  }

  \savedanchor{\RightAntennanortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@x=0.5\pgf@xa
    \pgf@y=0.5\pgf@ya
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from UserTerminal xxxxxxxxxxxxxxxxxxxx
  \inheritanchorborder[from=UserTerminal]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from UserTerminal xxxxxxxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % UserTerminal shape (even thought the northeast and southwest saved anchors
  % in the UserTerminal shape are different from ours).
  \inheritanchor[from=UserTerminal]{center}
  \inheritanchor[from=UserTerminal]{north}
  \inheritanchor[from=UserTerminal]{east}
  \inheritanchor[from=UserTerminal]{south}
  \inheritanchor[from=UserTerminal]{west}
  \inheritanchor[from=UserTerminal]{north east}
  \inheritanchor[from=UserTerminal]{north west}
  \inheritanchor[from=UserTerminal]{south west}
  \inheritanchor[from=UserTerminal]{south east}
  \inheritanchor[from=rectangle]{text}
  \anchor{antenna right}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
  }
  \anchor{antenna left}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{-\pgf@x}
  }
  \anchor{antenna center}{
    \northeast
    \pgfmathsetlength\pgf@y{0.8*\pgf@y}
    \pgfmathsetlength\pgf@x{0}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath.
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the background xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % The base of the antenna will be in the behindbackgroundpath while the
  % antennas will be in the backgroundpath. The main reason for this
  % separation is that this code here will be inherited in the
  % "BaseStation" shape that we will define later.
  \backgroundpath{
    % Scope for the antenna connector
    \begin{pgfscope}
      % Draw Antenna connector
      \pgfpathrectanglecorners
      {\AntennaConnectorsouthwest}
      {\AntennaConnectornortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}

    % Scope for the antennas
    \begin{pgfscope}
      % Draw the middle antenna
      \pgfpathrectanglecorners
      {\MiddleAntennasouthwest}
      {\MiddleAntennanortheast}

      % Draw the Left antenna
      \pgfpathrectanglecorners
      {\LeftAntennasouthwest}
      {\LeftAntennanortheast}

      % Draw the Right antenna
      \pgfpathrectanglecorners
      {\RightAntennasouthwest}
      {\RightAntennanortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx


% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx BaseStation Shape xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
\pgfdeclareshape{BaseStation}{

  % xxxxxxxxxx Define savedanchors xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  % Inherit all savedanchors from BaseStationSimple.
  \inheritsavedanchors[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxx Define savedanchors specific to the BaseStation shape xxxxxxxxxxx
  \savedanchor{\BaseAsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.5\pgf@ya
    \pgf@x=-0.2\pgf@xa
  }

  \savedanchor{\BaseAnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.2\pgf@xa
  }

  \savedanchor{\BaseBsoutheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=-0.05\pgf@ya
    \pgf@x=0.15\pgf@xa
  }

  \savedanchor{\BaseBnorthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.15\pgf@xa
  }

  \savedanchor{\BaseCsouthwest}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.15\pgf@ya
    \pgf@x=-0.1\pgf@xa
  }

  \savedanchor{\BaseCnortheast}{
    \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
    \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
    \pgf@y=0.30\pgf@ya
    \pgf@x=0.1\pgf@xa
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit anchor border from BaseStationSimple xxxxxxxxxxxxxxx
  \inheritanchorborder[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Inherit normal anchors from BaseStationSimple xxxxxxxxxxxxxx
  % We define the savedanchors "northeast" and "southwest". With these two
  % defined we can inherit code for the regular anchors from the
  % BaseStationSimple shape (even thought the northeast and southwest saved anchors
  % in the BaseStationSimple shape are different from ours)..
  \inheritanchor[from=BaseStationSimple]{center}
  \inheritanchor[from=BaseStationSimple]{north}
  \inheritanchor[from=BaseStationSimple]{east}
  \inheritanchor[from=BaseStationSimple]{south}
  \inheritanchor[from=BaseStationSimple]{west}
  \inheritanchor[from=BaseStationSimple]{north east}
  \inheritanchor[from=BaseStationSimple]{north west}
  \inheritanchor[from=BaseStationSimple]{south west}
  \inheritanchor[from=BaseStationSimple]{south east}
  \inheritanchor[from=BaseStationSimple]{antenna right}
  \inheritanchor[from=BaseStationSimple]{antenna left}
  \inheritanchor[from=BaseStationSimple]{antenna center}
  \inheritanchor[from=rectangle]{text}
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxxxx Draw the "behind background" xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
  \behindbackgroundpath{
    % Scope for the Base
    \begin{pgfscope}
      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseAsouthwest}
      {\BaseAnortheast}

      % Draw the middle base
      \pgfpathrectanglecorners
      {\BaseBsoutheast}
      {\BaseBnorthwest}

      % Draw the bottom base
      \pgfpathrectanglecorners
      {\BaseCsouthwest}
      {\BaseCnortheast}

      \pgfusepath{stroke,fill}
    \end{pgfscope}
  }
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

  % xxxxxxxx Inherit the background path from BaseStationSimple xxxxxxxxxxx
  \inheritbackgroundpath[from=BaseStationSimple]
  % xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
}
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxx END xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx
% xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "testbasestation.tex"
%%% TeX-PDF-mode: t
%%% End:

